The Optimal Power Flow Operator: Theory and Computation

Optimal power flow problems (OPFs) are mathematical programs used to determine how to distribute power over networks subject to network operation constraints and the physics of power flows. In this work, we take the view of treating an OPF problem as an operator which maps user demand to generated power, and allow the network parameters (such as generator and power flow limits) to take values in some admissible set. The contributions of this paper are to formalize this operator theoretic approach, define and characterize restricted parameter sets under which the mapping has a singleton output, independent binding constraints, and is differentiable. In contrast to related results in the optimization literature, we do not rely on introducing auxiliary slack variables. Indeed, our approach provides results that have a clear interpretation with respect to the power network under study. We further provide a closed-form expression for the Jacobian matrix of the OPF operator and describe how various derivatives can be computed using a recently proposed scheme based on homogenous self-dual embedding. Our framework of treating a mathematical program as an operator allows us to pose sensitivity and robustness questions from a completely different mathematical perspective and provide new insights into well studied problems.

==> OPFsensitivity.tex <==
\section{OPF Sensitivity}\label{sec:sen}
In this section we formally define the wort-case sensitivity of the DC-OPF and provide applications where its computation will be beneficial.
\subsection{Definition}
To study how the optimal generation reacts to the change in the load, we borrow the concept of sensitivity from \cite{Gri1990optimal,Yu2001sensitivity, Moh2014opf}. We first define the OPF sensitivity at a fixed point, and then extend to the worst-case sensitivity to take system contingency (operation points typically arising due to a system failure) into consideration.
\begin{definition}
For fixed $\{ \CM$, $\B$, $\f \}\in\setf$ and $\para\in\setparar$, 
consider a generator $i$ and a load $j$. The pair $(i,j)$ is said to be $C$-Lipschitz if
$\forall \delta>0$ and $\forall\alphavec,\betavec\in\setsl$ such that 
$|\alphavec_j-\betavec_j|\leq \delta$ and $\alphavec_k=\betavec_k (k\neq j)$,
we have $|\OPF_i(\alphavec)-\OPF_i(\betavec)|<C\delta$, where $\OPF_i(\cdot)$ denotes the $i$\textsuperscript{th} coordinate of the value of $\OPF(\cdot)$.
\end{definition}
\begin{definition}\label{df:op_sensitivity}
For fixed $\{ \CM$, $\B$, $\f \}\in\setf$ and $\para\in\setparar$,
the {\it fixed-point} sensitivity of generator $i$ with respective to load $j$ (i.e., bus $\nG+j$) is the minimal nonnegative value, denoted by $\sen_\ifromj$, such that
$(i,j)$ is a $C_\ifromj$-Lipschitz pair.
\end{definition}

\cref{df:op_sensitivity} assumes that all the network parameters including cost function, generator capacity and line capacity are fixed.
In real systems, as well as the  loads, the system parameters might also change with time. 
%For example,  system contingency, and maintenance, as well as other unexpected events \textsuperscript{{\color{red} citation needed}} will cause changes in \ja{\textbf{[do you want to metion toplogy changes here too?]}}.
For instance, if generator $i$ is shut down in an emergency, then this can be modeled by setting $\genulim_i$ and $\genllim_i$ to $0$ in the OPF problem in order to avoid misoperation 
\footnote{In fact, to satisfy \cref{A:limits}, $\genulim_i$ and $\genllim_i$ can be imagined to be set to $\epsilon_1,\epsilon_2$ for some small values, respectively.}.
Therefore, characterizing the worst-case sensitivity over all the possible operation points and system parameters will provide a uniform upper bound for the system sensitivity regardless of the real-time parameter, 
and also allow the system to tolerate generator contingency \cite{Wod2012power}. However, our current worst-case analysis is not over different graph topologies, so transmission contingency is not covered here.

\begin{definition}\label{df:wc_sensitivity}
The {\it worst-case} sensitivity of generator $i$ with respective to load $j$ (i.e., bus $\nG+j$) is
\begin{align}\label{eq:wcsen}
\wcsen_{\ifromj}:=\max\limits_{{\f}\in\setf}\max\limits_{\para\in\setparar(\f)} \sen_{\ifromj}.
\end{align}
\end{definition}

\begin{remark}
From the definition, both the operation-point or worst-case sensitivity can possibly {be unbounded above.}
\end{remark}
In \cref{sec:derivative}, we will define the derivative of $\OPF$ and provide conditions under which it exists and is smooth. This will pave the way to linking the $\OPF$ operator with worst-case sensitivity.

\subsection{Motivating Applications}\label{sec:app}
In this subsection, we will show why the metric of the worst-case sensitivity will play an important role in many recent applications. 
Specifically, we focus on three example problems: power system data privacy, real-time OPF error estimation and the range of LMPs.

\subsubsection{Power System Data Privacy}
%There is always some tension between the utilities and the research community. 
%As the development of the smart grid. More and more smart devices and cyber infrastructure have been playing an important role in %today's power systems. 
%While a great amount of electricity usage data become available, the growing concerns about data privacy also arise \cite{Sim2011analysis, Asg2017smart}.
%On the other hand, the advancement of data science motivates considerable research works driven by data.
%Both real or synthetic data are desired for data mining, cross validation and result publications \cite{Mor2006state, Bir2018power}.
Grid operators are often reluctant to disclose detailed power flow data as it may reveal sensitive information about clients and disclose vulnerabilities leading to security issues in the network. While a great amount of electricity usage data has become available, the growing concerns about data privacy also arise \cite{Sim2011analysis, Asg2017smart}. A  tradeoff between maintaining privacy and full disclosure, is  to provide some statistical summary data such as aggregated injections for specific geographical regions (vertex clusters) \cite{And2017disaggregation}.
In this setting we view the load vector $\sload$ as the private data, and suppose that the statistical summary is some function of all the bus injections $(\sgen,\sload)$.
Then $\sgen=\OPF(\sload)$ also contain certain amount of the privacy as it serves as a function of $\sload$.
We adopt {\it differential privacy} \cite{Dwo2006calibrating} as the metric to evaluate the privacy level.

Suppose $\mech(\sgen,\sload)$ is a (randomized) function of $(\sgen,\sload)$ in $\Real^r$. 
It is reasonable to assume that $\sgen$ is always chosen as the unique optimal solution to the OPF problem, i.e., $\sgen=\OPF(\sload)$.
Thereby $\mech(\sgen,\sload)=\mech(\OPF(\sload),\sload)$ is actually a function of $\sload $and we might simply write it as $\mech(\sload)$.
We introduced a modified definition of differential privacy in the context of power system data.
\begin{definition}
For $\Delta,\varrho>0$, the mechanism $\mech$ preserves $(\Delta,\varrho)$-differential privacy if and only if $\forall \data',\data''\in\setsl$ such that $\|\data'-\data''\|_0\leq1$ and $\|\data'-\data''\|_1\leq\Delta$, 
and $\forall \W\subseteq\Real^r$, we have
$\Prob\{\mech(\data')\in\W\}
\leq \exp(\varrho)\cdot\Prob\{\mech(\data'')\in\W\}.$
\end{definition}

The Laplace mechanism is one of the most commonly used mechanisms used to preserve differential pricy, and in our context, the Laplace mechanism can be characterized by the following lemma.
\begin{lemma}\label{lm:dp}
Let  $\tilde{\mech}(\sgen,\sload)$ be a deterministic function of $(\sgen,\sload)$ and we use $\tilde{\mech}(\sload)$ to denote $\tilde{\mech}(\OPF(\sload),\sload)$ for short. Suppose $\tilde{\mech}$ satisfies
$\forall \data',\data''\in\setsl$ such that $\|\data'-\data''\|_0\leq1$ and $\|\data'-\data''\|_1\leq\Delta$, 
we have 
$\|\tilde{\mech}(\data')-\tilde{\mech}(\data'')\|_1\leq \Delta_1.$

Then the mechanism $\mech=\tilde{\mech}+\dpnoises$, where all $\dpnoises_i$ are drawn 
from independent Laplace distributions $\Lap(\Delta_1/\varrho)$,
 preserves $(\Delta,\varrho)-$differential privacy.
\end{lemma}

Suppose $\tilde{\mech}$ is smooth and all the elements of the Jacobian matrix with respect to $\tilde{\mech}$ are upper bounded by a constant $U$.
Then by the chain rule, the worst-case sensitivity provides a natural upper bound for $\Delta_1$:
\begin{align*}
\Delta_1\leq \Big(1+\max\limits_{j\in[\nL]}\sum\limits_{i\in[\nG]}\wcsen_{\ifromj}\Big)Ur\Delta.
\end{align*}
Plugging the above upper bound in the expression for the parameter of the Laplace noise in
\cref{lm:dp} will preserve the $(\Delta,\varrho)-$differential privacy.
Informally, the sensitivity can be viewed as a metric evaluating how significantly a generator's change can reflect the change in the load.
In a system with higher worst-case sensitivity, even a tiny variance in the load can be amplified in the change of the optimal generation and such system might potentially leak more privacy while disclosing the statistical summary involving $\sgen$.

\subsubsection{Real-time OPF Error Estimation}
Solving AC OPF problems in real-time is an active area of interest \cite{Tan2017real, Ma2013distributed, Ber2017real}.
One of the main focuses of the real-time OPF algorithms is to track the optimal solution over a period of time while keeping the error between the optimal solution and the OFF algorithm outcome small. 
Estimating the solution error of the real-time OPF algorithm  provides valuable information for assessing the quality of an OPF algorithm and assessing how the network functions under different choices of algorithms. Take the state-of-art algorithm proposed by \cite{Tan2017real} as an example.
The authors used
\begin{align}\label{eq:tracking}
\frac{1}{T}\sum\limits_{t=1}^T \|\hat{\sgen}(t)-\sgen(t)\|
\end{align}
as the metric to measure the tracking performance, where $\hat{\sgen}$ and $\sgen$ are the algorithm outcome and the ground truth of the optimal solution.
%The time period is from $t=1$ to $T$. For simplicity, we assume the norm is the L2 norm, though in the original paper it is allowed to be weighted by an arbitrary positive definite matrix.
The upper bound of \eqref{eq:tracking} is also proposed in \cite{Tan2017real} to be of the form
\begin{align*}
\frac{1}{T}\sum\limits_{t=1}^T \|\hat{\sgen}(t)-\sgen(t)\|\leq \alpha\frac{1}{T}\sum\limits_{t=1}^T\|\sgen(t)-\sgen(t-1)\|+\beta
\end{align*}
where $\alpha$ and $\beta$ are the scalars determined by other parameters.
We notice that it might be difficult and unnatural to evaluate $\|\sgen(t)-\sgen(t-1)\|$ for 2 reasons. 
First, the value of the optimal solutions $\sgen(t)$ and $\sgen(t+1)$ are always unknown and so is their difference.
Second, the parameters in the OPF problem might also change time, so the value of $\|\sgen(t)-\sgen(t-1)\|$ is actually a variable of time.
Instead, it might be more natural to assume that $\|\sload(t)-\sload(t-1)\|$ is a relatively manageable and constant value as the usage of electricity usually does not change dramatically.
Our  worst-case sensitivity framework sheds light on the following relationship between the change in the optimal generation and the change in the load.
\begin{align}\label{eq:sl_to_sg}
\|\sgen(t)-\sgen(t-1)\|
\leq \max\limits_{j\in[\nL]}\sqrt{\sum\limits_{i\in[\nG]}(\wcsen_{\ifromj})^2}\|\sload(t)-\sload(t-1)\|.
\end{align}
If we view $\|\sload(t)-\sload(t-1)\|$ as a known or constant value, then the right hand side of \eqref{eq:sl_to_sg} is also known and does not change over time even if the cost function and other parameters of the OPF problem change.
It can also be seen from \eqref{eq:sl_to_sg} that in a highly sensitive system, the optimal generation might potentially fluctuate dramatically even if the loads change mildly, and it will make the real-time algorithm more difficult to track the optimal solution.
%However, it is important to point out that the real-time OPF problem usually adopts the AC model while our result only applies to the %DC model, \eqref{eq:sl_to_sg} should only serve as a rough estimation of the change in $\sgen$ over 2 consecutive time slots in the %AC model.

\subsubsection{Range of LMPs}
Locational marginal price (LMP) is the marginal cost of supplying the next increment of load at a specific bus \cite{Sha2003market}.
LMP is widely used in the control and operation of electricity markets as it characterizes the actual cost to generate and deliver the power.
Under the DC model, LMP at a given operating point can be explicitly expressed from KKT conditions \cite{Sha2003market},
and many literatures also propose the methods to forecast LMP in the near future \cite{Ji2013forecasting}.
It is also well known that LMP can be even higher than the price of the most expensive generator or be negative, since lie congestion also plays an important role in LMP,
and many papers also focus on the driver of those counter-intuitive LMPs \cite{Res2017understanding}.
We found that the worst-case sensitivity can provide a range for the LMP regardless of the operating point. 
Such result might be an alternative perspective to view LMP since such range can be regarded as the intrinsic LMP range determined by the system topology.
Specifically, the absolute value of LMP for load $j$ can be upper bound by
\begin{align*}
\sum\limits_{i\in[\nG]}\f_i\wcsen_{\ifromj}.
\end{align*}
Intuitively, if a system can potentially be highly sensitive, then it will be easier for the system to have extremely high or negative LMPs.
